Specification Mining for Smart Contracts with Trace Slicing and Predicate Abstraction

Smart contracts are computer programs running on blockchains to implement Decentralized Applications. The absence of contract specifications hinders routine tasks, such as contract understanding and testing. In this work, we propose a specification mining approach to infer contract specifications from past transaction histories. Our approach derives high-level behavioral automata of function invocations, accompanied by program invariants statistically inferred from the transaction histories. We implemented our approach as tool SMCON and evaluated it on eleven well-studied Azure benchmark smart contracts and six popular real-world DApp smart contracts. The experiments show that SMCON mines reasonably accurate specifications that can be used to enhance symbolic analysis of smart contracts achieving higher code coverage and up to 56% speedup, and facilitate DApp developers in maintaining high-quality documentation and test suites.

==> sections/SpecificationMining.tex <==
%!TEX root = ../main.tex
\section{Formal Analysis of Smart Contract}
\ca{Only the first and last paragraph mention smart contracts. This section is otherwise general and defines the spec.\ mining problem on execution traces. Either we keep this generic (and mention at the end that we apply this to smart contracts and what the specifics are in that context) or we clarify the points that are specific to SCs.}
\label{sec:analysis}
Smart contract consists of a set of state variables and a set of functions.
Let smart contract has $\mathit{n}$ state variables $\mathit{V}:\{v_1, \cdots, v_n\}$,
and $\mathit{k}$ functions $\mathit{M}:\{m_1,\cdots, m_k\}$.
Each function $\mathit{m}$ has a finite set of input parameters $\mathit{R_m}$.

\begin{definition}[Labeled Transition System (\lts)~\cite{beillahi2020behavioral}]
%	\textbf{().}
	A smart contract is a labeled transition system $(\mathit{S}, \mathit{s}_0, \Sigma, \delta)$
	where $\mathit{S}$ is a set of possibly-infinite states, $\mathit{s}_0 \in S$ is a initial state,
	$\Sigma$ is a possibly-infinite alphabet, and $\delta \subseteq \mathit{S} \times \Sigma \times
	\mathit{S}$ is a set of transitions.
	Let $\mathit{D_V}$ be the evaluation domains of $V$, we have $S \subset D_V$.
	Let $R$ be all possible parameters with evaluation domain $D_R$, we have $\Sigma \subset D_R$.
	$\delta(s_i, (m,$ \argumentvector $), s_j)$ represents a transition from a state $s_i$ to another state $s_j$ by calling  a method $m$ with \argumentvector, a vector of arguments over the parameters $R_m$.
	%		Clearly, $\mathit{S}=\mathit{D_{V_C}}$
	%		and $\Lambda = \mathit{D_{V_1}} \cup \cdots \cup \mathit{D_{V_m}}$.
\end{definition}

The \ltstext is a concrete system without abstraction.
Modeling smart contract behaviors using \lts will result an model with infinite concrete states or transitions.
Therefore, in order to obtain a compact representation of smart contract behaviors, we model smart contract as \efsmtext.
The definition is as follows.
\begin{definition}[Extended Finite State Machine (\efsm)~\cite{cheng1993automatic}]
\lts can be abstracted into an extended finite state machine with predicates over its states $\mathit{S}$, and its input parameters $\Sigma'$.
\efsm is a compact representation.
\efsm is defined as a 6-tuple $(Q, q_0, \Sigma', G, U, T)$ where
		\begin{itemize}
			\item $Q$ is a finite set of symbolic states under a predicate abstraction $\alpha$: $S \rightarrow Q$; $q_0 \in Q$ is the initial symbolic state.
			\item $\Sigma'$ is a finite alphabet and $\Sigma' = \cap_m \{R_m\}, \; m \in M$.
			\item $\mathit{G}$ is a set of \textit{guarding} function $\mathit{g_i}$ such that $g_i$: $D_V \times D_R \rightarrow \{\mathit{True}, \mathit{False}\}$,
			\item $\mathit{U}$ is a set of \textit{update} function $u_i$ such that $u_i$: $D_V \rightarrow D_V$,
			\item ${T}$ is a transition relation, ${T}:  {Q} \times \mathit{G} \times \Sigma \rightarrow {U} \times Q $.
		\end{itemize}
\end{definition}
To abstract \lts into \efsm precisely,
the key is precise predicate abstraction.
Predicate abstraction~\cite{clarke2000counterexample} is a function to create a partition of domain of data types.
For example, the widely used predicate abstraction for integer domain is \{$\mathit{neg}$, $\mathit{zero}$, $\mathit{pos}$\} which represent negative, zero and positive numbers respectively.
However, there could be many abstraction candidates.
In this work, we borrow the concept of minimal existential abstraction~\cite{chauhan2002automated}.
\begin{definition}[Minimal Existential Abstraction~\cite{chauhan2002automated}]
	\label{def:minimal}
	\efsm$=(Q, q_0, \Sigma', G, U, T)$ is the \minimalabstraction of \lts$=(\mathit{S}, \mathit{s}_0, \Sigma, \delta)$ with respect to $\alpha: S \rightarrow Q$ iff
	\begin{itemize}[leftmargin=*, label={}]
	\item (1) $\exists \; s_0\in S.\; \alpha(s_0)=q\; \Longleftrightarrow \; q = q_0$ and
	\item (2) $\exists \; (s_0, (m_i,$ \argumentvectori $), s_1), \cdots, (s_{n-1}, (m_j,$\argumentvectorj$), s_n) \in \delta.\; \alpha(s_0) = q_0 \land \alpha(s_1) = q_1 \land \cdots  \land \alpha(s_{n-1}) =  q_{n-1} \land \alpha(s_{n}) = q_{n} \; \Longleftrightarrow \; (q_0, \none,  R_i, \none, q_1), \cdots, (q_{n-1}, \none, R_j, \none, q_n) \in T$, where $(m_i,$ \argumentvectori $)$, $\cdots$, $(m_j,$\argumentvectorj$)$ is a sequence of function invocations.
	\end{itemize}
\end{definition}
The \minimalabstraction implies: (1) the initial concrete state can be mapped to initial symbolic state in the \efsmtext, and vice versa;
(2) every concrete path is preserved in the \efsmtext and every symbolic path in the \efsmtext has at least a corresponding concrete path.
%given a state predicate abstraction $\alpha$, \efsm contains neither spurious states nor spurious paths.

We now introduce the specification mining problem for smart contracts as follows.
\begin{definition}[Specification Mining Problem] \label{def:miningproblem}
	Given a contract's past transaction history, where all the happened contract behaviors are represented by \history,  mine an \efsm as the likely specification of smart contract.
\end{definition}


